SynDiff-AD: Improving Semantic Segmentation and End-to-End Autonomous Driving with Synthetic Data from Latent Diffusion Models

In recent years, significant progress has been made in collecting large-scale datasets to improve segmentation and autonomous driving models. These large-scale datasets are often dominated by common environmental conditions such as "Clear and Day" weather, leading to decreased performance in under-represented conditions like "Rainy and Night". To address this issue, we introduce SynDiff-AD, a novel data augmentation pipeline that leverages diffusion models (DMs) to generate realistic images for such subgroups. SynDiff-AD uses ControlNet-a DM that guides data generation conditioned on semantic maps-along with a novel prompting scheme that generates subgroup-specific, semantically dense prompts. By augmenting datasets with SynDiff-AD, we improve the performance of segmentation models like Mask2Former and SegFormer by up to 1.2% and 2.3% on the Waymo dataset, and up to 1.4% and 0.7% on the DeepDrive dataset, respectively. Additionally, we demonstrate that our SynDiff-AD pipeline enhances the driving performance of end-to-end autonomous driving models, like AIM-2D and AIM-BEV, by up to 20% across diverse environmental conditions in the CARLA autonomous driving simulator, providing a more robust model. We release our code and pipeline at https://github.com/UTAustin-SwarmLab/SynDiff-AD.

==> sections/experiments.tex <==



\section{Experiment}
\label{ss:experiments}

Our experiments aim to answer the following three questions to evaluate the efficacy of our approach.
\begin{enumerate}
    \item Does the proposed caption generation scheme using a large VLM like LLaVA impact the quality of the synthetic images over the test data subgroups (\ref{ss:cagimpact})?
    \item Does synthetic data improve the overall performance of both semantic segmentation and AD models (\ref{ss:perfoverall})?
    \item Does additional synthetic data improve the performance of the semantic segmentation models and AD over different sub-groups (\ref{ss:conditionexper})?
\end{enumerate}

\input{tables_latex/dataset_results}

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \textbf{Dataset} & \textbf{Model (Backbone)} & \textbf{Data} & \textbf{mIOU} & \textbf{mAcc}  & \textbf{mDICE} & \textbf{mF1} \\
%         \midrule
%          & Mask2Former (R50) & Real   & 46.7 & 59.3 & 57.4 & 59.5  \\
%          & Mask2Former (R50) & Real + Synth & 47.8 & 59.4 & 58.4 & 60.4 \\
%         Waymo & Mask2Former(Swin-T)& Real    & 50.2 & 61.1 & 60.0 & 62.2 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{51.5} & \textbf{62.1} & \textbf{61.9} & \textbf{64.1}  \\
%          & SegFormer (MIT-B3) & Real   & 45.4 & 53.6 & 55.2 & 61.6 \\
%          & SegFormer (MIT-B3) & Real + Synth    & 46.2 & 54.1 & 56.2 & 62.6  \\
%         \midrule
%          & Mask2Former (R50) & Real   & 51.5 & 61.5 & 63.5 & 66.8  \\
%          & Mask2Former (R50) & Real + Synth & 55.1 & 67.2 & 67.5 & 71.1  \\
%         DeepDrive & Mask2Former (Swin-T)& Real    & 57.2 & \textbf{70.5} & 69.8 & 69.8 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{58.6} & 70.2 & \textbf{70.7} & \textbf{74.5}  \\
%          & SegFormer (MIT-B3) & Real   & 53.9 & 64.3 & 66.1 & 69.6 \\
%          & SegFormer (MIT-B3)& Real + Synth    & 54.9 & 64.5 & 67.1 & 70.7  \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Models trained on augmented data outperform those trained on original data}. We show that the models fine-tuned on mixed datasets have increased performance over the standard metrics compared to their counterparts trained on original data. We set a new SOTA with Mask2Former Swin-T for AD segmentation.}
%     \label{tab:performance_per_npm}
%     \vspace{-1.2cm}
% \end{table}


\subsection{Datasets}
We conduct semantic segmentation experiments using two datasets: the \textbf{Waymo Open Dataset} \cite{sun2020scalability} and the \textbf{DeepDrive} dataset \cite{yu2020bdd100k}. The DeepDrive (BDD) dataset contains 7000 urban scene images annotated with semantic masks. captured across various locations in the United States 
Conversely, the Waymo Open Dataset comprises video segments captured by autonomous vehicles driving on roads, featuring multiple camera input streams. A subset of 37,618 images are annotated with semantic masks.  Additionally, we identify the operation design domain $\mathcal{Z}$ and semantic dimensions $\mathcal{Z}_{[0,1]}$ based on weather $\in \mathcal{Z}_0 = [\text{Rainy},\; \text{Clear},\; \text{Cloudy}]$ and time of day $\in \mathcal{Z}_1 = [\text{Dawn / Dusk},\; \text{Morning},\; \text{Night}] $. This results in 9 data subgroups for semantic segmentation tasks. 'Clear and Day' and 'Cloudy and Day' are over-represented data subgroups and comprise ($>80\%$) of the training data. 

For AD experiments, we curate a dataset with the expert driving policy in NEAT \cite{chitta2021neat} on CARLA. Our dataset is collected from an AV navigating three distinct towns along 15 routes, under various environmental conditions \cite{chitta2021neat}. The training data comprises images captured from three different camera views. Notably, a key deviation in our dataset collection compared to \cite{chitta2021neat} is that we fix weather conditions for each route to replicate real AD dataset collection. Finally, we test these models for 3 towns over 27 routes. For AD testing, the operation design domain $\mathcal{Z}$ and semantic dimensions $\mathcal{Z}_{[0,1]}$ is based on weather $\in \mathcal{Z}_0 = [\text{Rainy},\;\text{Clear},\;\text{Cloudy}]$ and time of day $\in \mathcal{Z}_1 = [\text{Twilight},\;\text{Morning},\;\text{Night}] $. 'Clear and Day' and 'Cloudy and Day' are over-represented data subgroups and comprise ($>50\%$) of training data.

\subsection{Experiment Details}

For the semantic segmentation task, we first finetune ControlNet on 8 A-5000 on both the Waymo and BDD datasets with VLM based text caption to generate subsequent synthetic samples. For BDD we generate $\sim 7000$ synthetic samples, and for Waymo we generate $\sim 36000$ samples (equal to size of respective datasets). Finally, we conduct our experiments over 3 segmentation models - Mask2Former \cite{cheng2022masked} with Swin-T \cite{liu2021swin} and Resnet-50 \cite{he2016deep} backbones and SegFormer \cite{xie2021segformer} with the MIT-B3 \cite{xie2021segformer} backbone. The segmentation models are pre-trained for $80000$ iterations on the original datasets and then finetuned for an additional $80000$ iterations using the augmented dataset or original dataset (baseline) with batch size 4. For the BDD dataset evaluation, we sampled and fixed 10 training images for the 'Cloudy and Dawn / Dusk' and 'Cloudy and Night' subgroups due to insufficient test samples (5 and 3 respectively).

\input{tables_latex/ad_performance}

For the AD tasks, we finetuned ControlNet to the dataset collected from CARLA. During training, the images and corresponding semantic masks are resized to a resolution of $512 \times 512$. For each task, finetuning occurs for 5 epochs over their respective datasets with a constant learning rate of $1 \times 10^{-5}$. During ControlNet inference, we swap the style as discussed in Algorithm~\ref{alg:ss_data_augmentation} to obtain the synthetic images for under-represented subgroups. The synthesis and finetuning are conducted over 8 A-5000 GPUs. Finally, we train NEAT \cite{chitta2021neat}, AIM-2D and AIM-BEV \cite{chitta2021neat}. These models when finetuned respectively with both datasets, have an equivalent number of gradient updates during training. Hence, we increase the batch size when training on augmented datasets. These experiments are conducted over a single A-5000 GPU. 


\subsection{Impact of Caption Generation (CaG)}
\label{ss:cagimpact}
We evaluate the quality of synthetic images generated by our proposed caption generation scheme using Frechet Distance (FD) \cite{heusel2017gans} which measures the distance between feature distributions of synthetic and original images. We compute FD scores between subgroup-specific distributions of synthetic and ground truth images using CLIP-VIT-L16 (dimension 768). We test the zero-shot synthetic data generated via text prompts augmented with VLM captions. Our results as seen Table~\ref{tab:performance_per_npm} show that CaG lowers FD scores, justifying the use of LLaVA to augment image captions for subsequent finetuning and image generation with ControlNet for segmentation and AD tasks.




\subsection{Effect of Finetuning on Final Performance}
\label{ss:perfoverall}
% \begin{figure}
%     \centering   
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth,height=0.8\linewidth]{/images/mask2former_r50_iou.png}
%         \caption{Mask2Former Resnet 50}
%         \label{fig:image3}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth,height=0.8\linewidth]{images/mask2former_swin_iou.png}
%         \caption{Mask2Former Swin-T}
%         \label{fig:image4}
%     \end{subfigure}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth,height=0.8\linewidth]{images/segformer_iou.png}
%         \caption{Segformer}
%         \label{fig:image5}
%     \end{subfigure}
%     \caption{\textbf{Performance (IoU) of different segmentation models finetuned over different datasets over different environment conditions.} We show modest performance gains especially over under-represented environmental test conditions.}
%     \label{fig:condition_results}
% \end{figure}

We analyze the performance of the finetuned segmentation models over metrics such as \textbf{mean Intersection over Union (mIoU)} and \textbf{mean F1 (mF1)} scores computed over all the semantic classes in the respective datasets. For AD models, we evaluate the models on the primary metric -- \textbf{Driving Score (DS)} -- which comprises \textbf{Route Completion (RC)} and \textbf{Infraction Score (IS)}.  \cite{chitta2021neat, chitta2022transfuser}. Route Completion (RC) refers to the fraction of the route completed by the vehicle, Infraction Score (IS) is inversely correlated with the violations made by the vehicle such as collisions, lane infractions, red light, and stop sign violations.

\input{tables_latex/dataset_ad_results}

\input{tables_latex/different_ad_performance}

As shown in Table~\ref{tab:performance_per_npm}, finetuning segmentation models on synthetic-augmented datasets improves performance. On Waymo, synthetic data boosts Mask2Former (Swin-T) by \textbf{+1.3 mIoU} and also enhances other models like Mask2Former (Resnet-50) and SegFormer (MIT-B3). Similar trends are seen on DeepDrive, with a notable \textbf{+3.6 mIoU} gain for Mask2Former (Resnet 50). We set a new SOTA with Mask2Former (Swin-T) on both the datasets.

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \scalebox{0.95}{
%     \begin{small}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sub-Group}} & \multirow{2}{*}{\textbf{Original}} & \multirow{2}{*}{\textbf{Synthetic}} & \textbf{Synthetic}  & \textbf{Synthetic} & \textbf{Synthetic} \\
%          & & & & \textbf{RST} & \textbf{CEQ} & \textbf{RST-CEQ}\\
%         \midrule
%          & Clear, Dawn/Dusk & 42.2 & 44.5 & 43.1 & 43.8 & \textbf{46.6}  \\
%          & Clear, Day       & 51.8 & \textbf{52.9} & 51.0 & 51.6 & 52.1 \\
%          & Clear, Night     & 33.6 & 36.4 & \textbf{39.3} & 34.2 & 33.9 \\
%          & Cloudy, Dawn/Dusk& 48.2 & 48.8 & 47.7 & \textbf{49.5} & 49.2   \\
%          Waymo& Cloudy, Day & \textbf{56.3} & 55.8 & \textbf{56.3} & 52.5 & 55.4 \\
%          & Cloudy, Night    & 38.3 & 38.1 & 35.9 & 37.5 & \textbf{39.9}  \\
%         & Rain, Dawn/Dusk   & 39.8 & \textbf{41.4} & 41.4 & 40.8 & 41.0   \\
%          & Rain, Day        & 50.7 & 50.7 & \textbf{52.7} & 51.5 & 50.8  \\
%          & Rain, Night      & 35.1 & 34.8 & 35.1 & \textbf{36.5} & 36.1   \\
%         \midrule
%          & Clear, Dawn/Dusk & 42.3 & 51.1 & \textbf{52.3} & 50.6 & 47.8  \\
%          & Clear, Day       & 56.7 & 57.5 & 57.2 & 55.9 & \textbf{57.8} \\
%          & Clear, Night     & 42.0 & \textbf{51.3} & 42.7 & 49.0 & 45.8 \\
%          & Cloudy, Dawn/Dusk& 40.8 & 42.4 & 42.6 & 35.8 & \textbf{44.3}   \\
%     DeepDrive& Cloudy, Day    & 52.2 & \textbf{60.4} & 55.8 & 57.0 & 59.6 \\
%          & Cloudy, Night    & 35.4 & 49.3 & 47.8 & 49.0 & \textbf{52.3} \\
%         & Rain, Dawn/Dusk   & 49.9 & \textbf{57.6} & 52.0 & 50.1 & 49.3   \\
%          & Rain, Day        & 54.8 & 56.6 & 56.0 & \textbf{57.7} & 55.2  \\
%          & Rain, Night      & 30.5 & 35.8 & 35.7 & 35.2 & \textbf{36.4}   \\
%         \bottomrule
%     \end{tabular}
%     \end{small}}
%     \caption{\textbf{Improved performance over different data subgroups with synthetic data augmentation}. We conduct an ablation study that constructs synthetic datasets using three approaches - RST, CEQ, and RST - CEQ. RST datasets comprise images from a fine-tuned ControlNet that equally samples rare subgroups during training. CEQ datasets are sampled so that the synthetic dataset's semantic class distribution is uniform. RST-CEQ incorporates both these strategies.}\label{tab:performance_per_subgroup_sem}
%     \vspace{-1.0 cm}
% \end{table}

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \scalebox{0.95}{
%     \begin{small}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sub-Group}} & \multirow{2}{*}{\textbf{Original}} & \multirow{2}{*}{\textbf{Synthetic}} & \textbf{Synthetic}  & \textbf{Synthetic} & \textbf{Synthetic} \\
%          & & & & \textbf{RST} & \textbf{CEQ} & \textbf{RST-CEQ}\\
%         \midrule
%          & Clear, Dawn/Dusk & 42.2 & 44.5 & 43.1 & 43.8 & \textbf{46.6}  \\
%          & Clear, Day       & 51.8 & \textbf{52.9} & 51.0 & 51.6 & 52.1 \\
%          & Clear, Night     & 33.6 & 36.4 & \textbf{39.3} & 34.2 & 33.9 \\
%          & Cloudy, Dawn/Dusk& 48.2 & 48.8 & 47.7 & \textbf{49.5} & 49.2   \\
%          Waymo& Cloudy, Day & \textbf{56.3} & 55.8 & \textbf{56.3} & 52.5 & 55.4 \\
%          & Cloudy, Night    & 38.3 & 38.1 & 35.9 & 37.5 & \textbf{39.9}  \\
%         & Rain, Dawn/Dusk   & 39.8 & \textbf{41.4} & 41.4 & 40.8 & 41.0   \\
%          & Rain, Day        & 50.7 & 50.7 & \textbf{52.7} & 51.5 & 50.8  \\
%          & Rain, Night      & 35.1 & 34.8 & 35.1 & \textbf{36.5} & 36.1   \\
%         \midrule
%          & Clear, Dawn/Dusk & 42.3 & 51.1 & \textbf{52.3} & 50.6 & 47.8  \\
%          & Clear, Day       & 56.7 & 57.5 & 57.2 & 55.9 & \textbf{57.8} \\
%          & Clear, Night     & 42.0 & \textbf{51.3} & 42.7 & 49.0 & 45.8 \\
%          & Cloudy, Dawn/Dusk& 40.8 & 42.4 & 42.6 & 35.8 & \textbf{44.3}   \\
%     DeepDrive& Cloudy, Day    & 52.2 & \textbf{60.4} & 55.8 & 57.0 & 59.6 \\
%          & Cloudy, Night    & 35.4 & 49.3 & 47.8 & 49.0 & \textbf{52.3} \\
%         & Rain, Dawn/Dusk   & 49.9 & \textbf{57.6} & 52.0 & 50.1 & 49.3   \\
%          & Rain, Day        & 54.8 & 56.6 & 56.0 & \textbf{57.7} & 55.2  \\
%          & Rain, Night      & 30.5 & 35.8 & 35.7 & 35.2 & \textbf{36.4}   \\
%         \bottomrule
%     \end{tabular}
%     \end{small}}
%     \caption{\textbf{Improved performance over different data subgroups with synthetic data augmentation}. We conduct an ablation study that constructs synthetic datasets using three approaches - RST, CEQ, and RST - CEQ. RST datasets comprise images from a fine-tuned ControlNet that equally samples rare subgroups during training. CEQ datasets are sampled so that the synthetic dataset's semantic class distribution is uniform. RST-CEQ incorporates both these strategies.}\label{tab:performance_per_subgroup_sem}
%     \vspace{-1.0 cm}
% \end{table}

For AD experiments, we observe improved DS performance in AIM-2D (\textbf{21.64 $\to$ 34.36}) and AIM-BEV (\textbf{28.61 $\to$ 35.86}) trained on the augmented dataset. This improvement is primarily due to an increase in IS, as the RC performance is capped by the expert's performance due to the lack of data support. This indicates robustness in the performance of the AV, as it is penalized less for violating traffic rules or colliding with objects in the scene. In the case of NEAT which makes waypoint predictions using three camera views, we observe an overall degradation in driving performance. We think that is due to the lack of spatial consistency in synthetic images for different camera views.

In conclusion, synthetic images aid in learning performant models as these conduct context-sensitive augmentations over the original ground truth data. This enables better generalization to different visual elements across all subgroups. 

\subsection{Effect of Finetuning on Condition-Specific Performance}
\label{ss:conditionexper}
Finally, we discuss the impact of synthetic data generated using our approach on the final subgroup-specific performance of the model through two key tables: Table~\ref{tab:performance_per_subgroup_sem} for semantic segmentation tasks and Table~\ref{tab:performance_per_subgroup_sem_ad}.

For semantic segmentation, an equal number of synthetic data samples are generated for each data subgroup across all datasets. The best-performing semantic segmentation model, Mask2Former, is finetuned on both the original datasets and the augmented datasets that include synthetic data. The results in Table~\ref{tab:performance_per_subgroup_sem} demonstrate that the models finetuned on the augmented datasets consistently outperform those trained on the original datasets alone, across all subgroups. This suggests that the addition of synthetic data enhances the model's ability to generalize and improve performance on under-represented data subgroups. 

\input{figures_latex/examples}

Finally, we report the per subgroup test performance of various AD models in Table~\ref{tab:performance_per_subgroup_sem_ad}. Here, the synthetic data is generated for all camera views across an entire route. The performance of various AD models is evaluated after being trained on the original dataset and the augmented dataset respectively. We see noticeable improvements in the driving score of AD models AIM-2D and AIM-BEV when trained with synthetic data augmentations using \ours \space on all data subgroups. In contrast, we observe a degradation in the performance of NEAT with synthetic data augmentations which is likely due to the reasons mentioned in Section~\ref{ss:perfoverall}.

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \textbf{Dataset} & \textbf{Model (Backbone)} & \textbf{Data} & \textbf{mIOU} & \textbf{mAcc}  & \textbf{mDICE} & \textbf{mF1} \\
%         \midrule
%          & Mask2Former (R50) & Real   & 46.7 & 59.3 & 57.4 & 59.5  \\
%          & Mask2Former (R50) & Real + Synth & 47.6 & 58.2 & 58.1 & 60.2 \\
%         Waymo & Mask2Former(Swin-T)& Real    & 50.2 & 61.1 & 60.0 & 62.2 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{51.5} & \textbf{62.1} & \textbf{61.9} & \textbf{64.1}  \\
%          & SegFormer (MIT-B3) & Real   & 45.4 & 53.6 & 55.2 & 61.6 \\
%          & SegFormer (MIT-B3) & Real + Synth    & 45.6 & 53.9 & 55.6 & 62.1  \\
%         \midrule
%          & Mask2Former (R50) & Real   & 51.5 & 61.5 & 63.5 & 66.8  \\
%          & Mask2Former (R50) & Real + Synth & 55.1 & 67.2 & 67.5 & 71.1  \\
%         DeepDrive & Mask2Forvmer (Swin-T)& Real    & 57.2 & \textbf{70.5} & 69.8 & 69.8 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{58.6} & 70.2 & \textbf{70.7} & \textbf{74.5}  \\
%          & SegFormer (MIT-B3) & Real   & 53.9 & 64.3 & 66.1 & 69.6 \\
%          & SegFormer (MIT-B3)& Real + Synth    & 54.9 & 64.5 & 67.1 & 70.7  \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Comprehensive Performance Comparison Across Models and finetuning datasets}. We show that the models fine-tuned on mixed datasets have marginal performance improvements over the standard metrics. Note that M2Former is a short hand for Mask2Former.}
%     \label{tab:performance_per_npm}
% \end{table}



==> sections/experiments_v2_harsh.tex <==




\section{Experiments}
\label{ss:experiments}

We evaluate the efficacy of the synthetic data generated with \ours \space on segmentation and AD. We now outline the datasets, experiment setup, and evaluation metrics.

\input{tables_latex/dataset_results}

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \textbf{Dataset} & \textbf{Model (Backbone)} & \textbf{Data} & \textbf{mIOU} & \textbf{mAcc}  & \textbf{mDICE} & \textbf{mF1} \\
%         \midrule
%          & Mask2Former (R50) & Real   & 46.7 & 59.3 & 57.4 & 59.5  \\
%          & Mask2Former (R50) & Real + Synth & 47.8 & 59.4 & 58.4 & 60.4 \\
%         Waymo & Mask2Former(Swin-T)& Real    & 50.2 & 61.1 & 60.0 & 62.2 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{51.5} & \textbf{62.1} & \textbf{61.9} & \textbf{64.1}  \\
%          & SegFormer (MIT-B3) & Real   & 45.4 & 53.6 & 55.2 & 61.6 \\
%          & SegFormer (MIT-B3) & Real + Synth    & 46.2 & 54.1 & 56.2 & 62.6  \\
%         \midrule
%          & Mask2Former (R50) & Real   & 51.5 & 61.5 & 63.5 & 66.8  \\
%          & Mask2Former (R50) & Real + Synth & 55.1 & 67.2 & 67.5 & 71.1  \\
%         DeepDrive & Mask2Former (Swin-T)& Real    & 57.2 & \textbf{70.5} & 69.8 & 69.8 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{58.6} & 70.2 & \textbf{70.7} & \textbf{74.5}  \\
%          & SegFormer (MIT-B3) & Real   & 53.9 & 64.3 & 66.1 & 69.6 \\
%          & SegFormer (MIT-B3)& Real + Synth    & 54.9 & 64.5 & 67.1 & 70.7  \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Models trained on augmented data outperform those trained on original data}. We show that the models fine-tuned on mixed datasets have increased performance over the standard metrics compared to their counterparts trained on original data. We set a new SOTA with Mask2Former Swin-T for AD segmentation.}
%     \label{tab:performance_per_npm}
%     \vspace{-1.2cm}
% \end{table}


\subsection{Datasets}
We conduct semantic segmentation experiments using two datasets: the \textbf{Waymo Open Dataset} \cite{sun2020scalability} and the \textbf{DeepDrive} dataset \cite{yu2020bdd100k}. The DeepDrive (BDD) dataset contains 7000 urban scene images annotated with semantic masks. captured across various locations in the United States 
Conversely, the Waymo Open Dataset comprises video segments captured by autonomous vehicles driving on roads, featuring multiple camera input streams. A subset of 37,618 images are annotated with semantic masks.  Additionally, we identify the set of all subgroups $\mathcal{Z}$ and semantic dimensions $\mathcal{Z}_{[0,1]}$ based on weather $\in \mathcal{Z}_0 = [\text{Rainy},\; \text{Clear},\; \text{Cloudy}]$ and time of day $\in \mathcal{Z}_1 = [\text{Dawn / Dusk},\; \text{Morning},\; \text{Night}] $. This results in 9 data subgroups for semantic segmentation tasks. ``Clear and Day'' and ``Cloudy and Day'' are over-represented data subgroups and comprise ($>80\%$) of the training data. 

For AD experiments, we curate a dataset with the expert driving policy in NEAT \cite{chitta2021neat} on CARLA. Our dataset is collected from an AV navigating three distinct towns along 15 routes, under various environmental conditions \cite{chitta2021neat}. The training data comprises images captured from three different camera views. Notably, a key deviation in our dataset collection compared to \cite{chitta2021neat} is that we fix weather conditions for each route to replicate real AD dataset collection. Finally, we test these models for 3 towns over 27 routes. For AD testing, the operation design domain $\mathcal{Z}$ and semantic dimensions $\mathcal{Z}_{[0,1]}$ is based on weather $\in \mathcal{Z}_0 = [\text{Rainy},\;\text{Clear},\;\text{Cloudy}]$ and time of day $\in \mathcal{Z}_1 = [\text{Twilight},\;\text{Morning},\;\text{Night}] $. ``Clear and Day'' and ``Cloudy and Day'' are over-represented data subgroups and comprise ($>50\%$) of training data.

\subsection{Experiment Details}
                          
For the semantic segmentation task, we first finetune ControlNet on 8 A-5000 on both the Waymo and BDD datasets with VLM based text caption to generate subsequent synthetic samples. For BDD we generate $\sim 7000$ synthetic samples, and for Waymo we generate $\sim 36000$ samples (equal to size of respective datasets). Finally, we conduct our experiments over 3 segmentation models - Mask2Former \cite{cheng2022masked} with Swin-T \cite{liu2021swin} and Resnet-50 \cite{he2016deep} backbones and SegFormer \cite{xie2021segformer} with the MIT-B3 \cite{xie2021segformer} backbone. The segmentation models are pre-trained for $80000$ iterations on the original datasets and then finetuned for an additional $80000$ iterations using the augmented dataset or original dataset (baseline) with batch size 4. 

% For the BDD dataset evaluation, we sampled and fixed 10 training images for the ``Cloudy and Dawn / Dusk'' and ``Cloudy and Night'' subgroups due to insufficient test samples (5 and 3 respectively).

\input{tables_latex/ad_performance}

For the AD tasks, we finetuned ControlNet to the dataset collected from CARLA. During training, the images and corresponding semantic masks are resized to a resolution of $512 \times 512$. For each task, finetuning occurs for 5 epochs over their respective datasets with a constant learning rate of $1 \times 10^{-5}$. During ControlNet inference, we swap the style as discussed in Algorithm~\ref{alg:ss_data_augmentation} to obtain the synthetic images for under-represented subgroups. The synthesis and finetuning are conducted over 8 A-5000 GPUs. Finally, we train NEAT \cite{chitta2021neat}, AIM-2D and AIM-BEV \cite{chitta2021neat}. These models when finetuned respectively with both datasets, have an equivalent number of gradient updates during training. Hence, we increase the batch size when training on augmented datasets. These experiments are conducted over a single A-5000 GPU. 

\subsection{Metrics}

We analyze the performance of the finetuned segmentation models over metrics such as \textbf{mean Intersection over Union (mIoU)} and \textbf{mean F1 (mF1)} scores computed over all the semantic classes in the respective datasets. For AD models, we evaluate the models on the primary metric -- \textbf{Driving Score (DS)} -- which comprises \textbf{Route Completion (RC)} and \textbf{Infraction Score (IS)}.  \cite{chitta2021neat, chitta2022transfuser}. Route Completion (RC) refers to the fraction of the route completed by the vehicle, Infraction Score (IS) is inversely correlated with the violations made by the vehicle such as collisions, lane infractions, red light, and stop sign violations.


\section{Results and Discussions}
Our experiments aim to answer the following three questions to evaluate the efficacy of our approach.
\begin{enumerate}
    \item Does the proposed caption generation scheme using a large VLM like LLaVA impact the quality of the synthetic images over the test data subgroups?
    \item Does synthetic data improve the overall performance of both semantic segmentation and AD models?
    \item Does additional synthetic data improve the performance of the semantic segmentation models and AD over different sub-groups?
\end{enumerate}

\input{tables_latex/dataset_ad_results}
\input{tables_latex/different_ad_performance}


\textbf{Research Question 1:}
\label{ss:cagimpact}
We evaluate the quality of synthetic images generated by our proposed caption generation scheme using Frechet Distance (FD) \cite{heusel2017gans} which measures the distance between feature distributions of synthetic and original images. We compute FD scores between subgroup-specific distributions of synthetic and ground truth images using CLIP-VIT-L16 (dimension 768). We test the zero-shot synthetic data generated via text prompts augmented with VLM captions. Our results as seen Table~\ref{tab:performance_per_npm} show that CaG lowers FD scores, justifying the use of LLaVA to augment image captions for subsequent finetuning and image generation with ControlNet for segmentation and AD tasks.


\input{figures_latex/examples}

\textbf{Research Question 2:}
\label{ss:perfoverall}
As shown in Table~\ref{tab:performance_per_npm}, finetuning segmentation models on synthetic-augmented datasets improves performance. On Waymo, synthetic data boosts Mask2Former (Swin-T) by \textbf{+1.3 mIoU} and also enhances other models like Mask2Former (Resnet-50) and SegFormer (MIT-B3). Similar trends are seen on DeepDrive, with a notable \textbf{+3.6 mIoU} gain for Mask2Former (Resnet 50). We set a new SOTA with Mask2Former (Swin-T) on both the datasets.


% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \scalebox{0.95}{
%     \begin{small}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sub-Group}} & \multirow{2}{*}{\textbf{Original}} & \multirow{2}{*}{\textbf{Synthetic}} & \textbf{Synthetic}  & \textbf{Synthetic} & \textbf{Synthetic} \\
%          & & & & \textbf{RST} & \textbf{CEQ} & \textbf{RST-CEQ}\\
%         \midrule
%          & Clear, Dawn/Dusk & 42.2 & 44.5 & 43.1 & 43.8 & \textbf{46.6}  \\
%          & Clear, Day       & 51.8 & \textbf{52.9} & 51.0 & 51.6 & 52.1 \\
%          & Clear, Night     & 33.6 & 36.4 & \textbf{39.3} & 34.2 & 33.9 \\
%          & Cloudy, Dawn/Dusk& 48.2 & 48.8 & 47.7 & \textbf{49.5} & 49.2   \\
%          Waymo& Cloudy, Day & \textbf{56.3} & 55.8 & \textbf{56.3} & 52.5 & 55.4 \\
%          & Cloudy, Night    & 38.3 & 38.1 & 35.9 & 37.5 & \textbf{39.9}  \\
%         & Rain, Dawn/Dusk   & 39.8 & \textbf{41.4} & 41.4 & 40.8 & 41.0   \\
%          & Rain, Day        & 50.7 & 50.7 & \textbf{52.7} & 51.5 & 50.8  \\
%          & Rain, Night      & 35.1 & 34.8 & 35.1 & \textbf{36.5} & 36.1   \\
%         \midrule
%          & Clear, Dawn/Dusk & 42.3 & 51.1 & \textbf{52.3} & 50.6 & 47.8  \\
%          & Clear, Day       & 56.7 & 57.5 & 57.2 & 55.9 & \textbf{57.8} \\
%          & Clear, Night     & 42.0 & \textbf{51.3} & 42.7 & 49.0 & 45.8 \\
%          & Cloudy, Dawn/Dusk& 40.8 & 42.4 & 42.6 & 35.8 & \textbf{44.3}   \\
%     DeepDrive& Cloudy, Day    & 52.2 & \textbf{60.4} & 55.8 & 57.0 & 59.6 \\
%          & Cloudy, Night    & 35.4 & 49.3 & 47.8 & 49.0 & \textbf{52.3} \\
%         & Rain, Dawn/Dusk   & 49.9 & \textbf{57.6} & 52.0 & 50.1 & 49.3   \\
%          & Rain, Day        & 54.8 & 56.6 & 56.0 & \textbf{57.7} & 55.2  \\
%          & Rain, Night      & 30.5 & 35.8 & 35.7 & 35.2 & \textbf{36.4}   \\
%         \bottomrule
%     \end{tabular}
%     \end{small}}
%     \caption{\textbf{Improved performance over different data subgroups with synthetic data augmentation}. We conduct an ablation study that constructs synthetic datasets using three approaches - RST, CEQ, and RST - CEQ. RST datasets comprise images from a fine-tuned ControlNet that equally samples rare subgroups during training. CEQ datasets are sampled so that the synthetic dataset's semantic class distribution is uniform. RST-CEQ incorporates both these strategies.}\label{tab:performance_per_subgroup_sem}
%     \vspace{-1.0 cm}
% \end{table}

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \scalebox{0.95}{
%     \begin{small}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sub-Group}} & \multirow{2}{*}{\textbf{Original}} & \multirow{2}{*}{\textbf{Synthetic}} & \textbf{Synthetic}  & \textbf{Synthetic} & \textbf{Synthetic} \\
%          & & & & \textbf{RST} & \textbf{CEQ} & \textbf{RST-CEQ}\\
%         \midrule
%          & Clear, Dawn/Dusk & 42.2 & 44.5 & 43.1 & 43.8 & \textbf{46.6}  \\
%          & Clear, Day       & 51.8 & \textbf{52.9} & 51.0 & 51.6 & 52.1 \\
%          & Clear, Night     & 33.6 & 36.4 & \textbf{39.3} & 34.2 & 33.9 \\
%          & Cloudy, Dawn/Dusk& 48.2 & 48.8 & 47.7 & \textbf{49.5} & 49.2   \\
%          Waymo& Cloudy, Day & \textbf{56.3} & 55.8 & \textbf{56.3} & 52.5 & 55.4 \\
%          & Cloudy, Night    & 38.3 & 38.1 & 35.9 & 37.5 & \textbf{39.9}  \\
%         & Rain, Dawn/Dusk   & 39.8 & \textbf{41.4} & 41.4 & 40.8 & 41.0   \\
%          & Rain, Day        & 50.7 & 50.7 & \textbf{52.7} & 51.5 & 50.8  \\
%          & Rain, Night      & 35.1 & 34.8 & 35.1 & \textbf{36.5} & 36.1   \\
%         \midrule
%          & Clear, Dawn/Dusk & 42.3 & 51.1 & \textbf{52.3} & 50.6 & 47.8  \\
%          & Clear, Day       & 56.7 & 57.5 & 57.2 & 55.9 & \textbf{57.8} \\
%          & Clear, Night     & 42.0 & \textbf{51.3} & 42.7 & 49.0 & 45.8 \\
%          & Cloudy, Dawn/Dusk& 40.8 & 42.4 & 42.6 & 35.8 & \textbf{44.3}   \\
%     DeepDrive& Cloudy, Day    & 52.2 & \textbf{60.4} & 55.8 & 57.0 & 59.6 \\
%          & Cloudy, Night    & 35.4 & 49.3 & 47.8 & 49.0 & \textbf{52.3} \\
%         & Rain, Dawn/Dusk   & 49.9 & \textbf{57.6} & 52.0 & 50.1 & 49.3   \\
%          & Rain, Day        & 54.8 & 56.6 & 56.0 & \textbf{57.7} & 55.2  \\
%          & Rain, Night      & 30.5 & 35.8 & 35.7 & 35.2 & \textbf{36.4}   \\
%         \bottomrule
%     \end{tabular}
%     \end{small}}
%     \caption{\textbf{Improved performance over different data subgroups with synthetic data augmentation}. We conduct an ablation study that constructs synthetic datasets using three approaches - RST, CEQ, and RST - CEQ. RST datasets comprise images from a fine-tuned ControlNet that equally samples rare subgroups during training. CEQ datasets are sampled so that the synthetic dataset's semantic class distribution is uniform. RST-CEQ incorporates both these strategies.}\label{tab:performance_per_subgroup_sem}
%     \vspace{-1.0 cm}
% \end{table}



For AD experiments, we observe improved DS performance in AIM-2D (\textbf{21.64 $\to$ 34.36}) and AIM-BEV (\textbf{28.61 $\to$ 35.86}) trained on the augmented dataset. This improvement is primarily due to an increase in IS, as the RC performance is capped by the expert's performance due to lack of data support. This indicates robustness in the performance of the AV, as it is penalized less for violating traffic rules or colliding with objects in the scene. In the case of NEAT which makes waypoint predictions using three camera views, we observe an overall degradation in driving performance. We think that is due to the lack of spatial consistency in synthetic images for different camera views.

In conclusion, synthetic images aid in learning performant models as these conduct context-sensitive augmentations over the original ground truth data. This enables better generalization to different visual elements across all subgroups. 


\textbf{Research Question 3:}
% \label{ss:conditionexper}
Finally, we discuss the impact of synthetic data generated using our approach on the final subgroup-specific performance of the model through two key tables: Table~\ref{tab:performance_per_subgroup_sem} for semantic segmentation tasks and Table~\ref{tab:performance_per_subgroup_sem_ad}.

For semantic segmentation, an equal number of synthetic data samples are generated for each data subgroup across all datasets. The best-performing semantic segmentation model, Mask2Former, is finetuned on both the original datasets and the augmented datasets that include synthetic data. The results in Table~\ref{tab:performance_per_subgroup_sem} demonstrate that the models finetuned on the augmented datasets consistently outperform those trained on the original datasets alone, across all subgroups. This suggests that the addition of synthetic data enhances the model's ability to generalize and improve performance on under-represented data subgroups. 

Finally, we report the per subgroup test performance of various AD models in Table~\ref{tab:performance_per_subgroup_sem_ad}. Here, the synthetic data is generated for all camera views across an entire route. The performance of various AD models is evaluated after being trained on the original dataset and the augmented dataset respectively. We see noticeable improvements in the driving score of AD models AIM-2D and AIM-BEV when trained with synthetic data augmentations using \ours \space on all data subgroups. In contrast, we observe a degradation in the performance of NEAT with synthetic data augmentations which is likely due to the reasons mentioned in Section~\ref{ss:perfoverall}.

% \begin{table}
%     \centering
%     \captionsetup{justification=raggedright, singlelinecheck=false}
%     \begin{tabular}{@{}ccccccc@{}}
%         \toprule
%         \textbf{Dataset} & \textbf{Model (Backbone)} & \textbf{Data} & \textbf{mIOU} & \textbf{mAcc}  & \textbf{mDICE} & \textbf{mF1} \\
%         \midrule
%          & Mask2Former (R50) & Real   & 46.7 & 59.3 & 57.4 & 59.5  \\
%          & Mask2Former (R50) & Real + Synth & 47.6 & 58.2 & 58.1 & 60.2 \\
%         Waymo & Mask2Former(Swin-T)& Real    & 50.2 & 61.1 & 60.0 & 62.2 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{51.5} & \textbf{62.1} & \textbf{61.9} & \textbf{64.1}  \\
%          & SegFormer (MIT-B3) & Real   & 45.4 & 53.6 & 55.2 & 61.6 \\
%          & SegFormer (MIT-B3) & Real + Synth    & 45.6 & 53.9 & 55.6 & 62.1  \\
%         \midrule
%          & Mask2Former (R50) & Real   & 51.5 & 61.5 & 63.5 & 66.8  \\
%          & Mask2Former (R50) & Real + Synth & 55.1 & 67.2 & 67.5 & 71.1  \\
%         DeepDrive & Mask2Forvmer (Swin-T)& Real    & 57.2 & \textbf{70.5} & 69.8 & 69.8 \\
%          & Mask2Former (Swin-T)& Real + Synth     & \textbf{58.6} & 70.2 & \textbf{70.7} & \textbf{74.5}  \\
%          & SegFormer (MIT-B3) & Real   & 53.9 & 64.3 & 66.1 & 69.6 \\
%          & SegFormer (MIT-B3)& Real + Synth    & 54.9 & 64.5 & 67.1 & 70.7  \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Comprehensive Performance Comparison Across Models and finetuning datasets}. We show that the models fine-tuned on mixed datasets have marginal performance improvements over the standard metrics. Note that M2Former is a short hand for Mask2Former.}
%     \label{tab:performance_per_npm}
% \end{table}



==> sections/intro.tex <==
\section{Introduction}

Over the last decade, Autonomous Driving (AD) has experienced remarkable advancements with vehicle fleets collecting terabytes (TBs) of driving data each day. This process has expanded data availability at an unprecedented scale. This availability has propelled the development of deep neural networks (DNNs) with millions of parameters for tasks like object detection, semantic segmentation, and end-to-end (E2E) AD.

\input{figures_latex/introduction_figure}
Despite this progress, we observe that the majority of the collected samples are biased toward certain weather conditions. For example, we find that the \textbf{Waymo Open} dataset \cite{sun2020scalability} and the \textbf{DeepDrive} dataset \cite{yu2020bdd100k} have 65\% and 70\% samples in sunny and clear weather conditions. Such over-representation in AD datasets affects the performance of segmentation \cite{kerim2022semantic} and planning tasks \cite{pmlr-v205-agarwal23b, agarwal2023robust} on rare dataset subgroups such as rainy, cloudy weather conditions. A natural solution to this problem is to collect additional driving data for rare subgroups \cite{akcin2023data}. However, the subsequent manual labeling process for segmentation and E2E AD is expensive and time-consuming.

To address these challenges, we propose \ours, a novel pipeline to generate realistic data for under-represented subgroups, to augment the existing AD datasets. Our key insight in \ours \space is to leverage the vast improvements in text-to-image controlled generation such as  \cite{rombach2021highresolution, ramesh2022hierarchical} to generate variants of the existing dataset samples while preserving their semantic structure. This mitigates the need for manual labeling for semantic segmentation and E2E AD. Our approach is detailed in Fig.~\ref{fig:intro_fig}. We first identify the under-represented subgroups in any dataset (Step 1) and use a finetuned ControlNet \cite{zhang2023adding}, a latent diffusion model (LDM), to synthesize samples for under-represented subgroups from the corresponding ground truth label \harsh{what label?} of over-represented subgroups in the dataset (Step 2). Finally, we augment the datasets with the generated samples to finetune the segmentation and E2E AD models (Step 3). We emphasize that our approach requires \textbf{zero human intervention.} 

Our key contributions are summarised as follows:
\begin{enumerate}
\item We propose \ours, a conditional LDM-based approach that generates samples for under-represented subgroups in a dataset. \ours \space transforms samples from the over-represented subgroups without disturbing their semantic structure. 

\item Inspired by textual inversion, we introduce a novel prompting scheme for data augmentation that is based on captions obtained from LLaVA \harsh{add reference}, a vision-language captioning model. We surgically transform these descriptions to steer the generation process in \ours \space towards the under-represented subgroups.

% we introduce a novel prompting scheme that directs the generation process in \ours towards the under-represented subgroups. We surgically transform the descriptions of images from the over-represented subgroups obtained from a LLaVA, a vision-language captioning model, to represent scenarios from the under-represented subgroups.

\item We empirically demonstrate that finetuning semantic segmentation and AD models on augmented datasets improves their performance across all subgroups. 
\end{enumerate}

% \item Finally, we are the first to show that we can augment autonomous driving datasets with a blend of real and synthetic images without the need for additional expert data. Autonomous driving models fine-tuned on augmented datasets showed improved driving performance across various test subgroups.

% \item We propose fine-tuning ControlNet with a text description of an image generated by a vision-language captioning model, LLaVA. Our experiments reveal that this approach improves the quality of images generated for downstream synthesis.

% \item Inspired by textual inversion, we propose fine-tuning ControlNet to generate synthetic data for different data subgroups through style prompting. To achieve this, we integrate captions generated by the vision captioning model LLaVA and identify data subgroups as a stylistic guide for fine-tuning ControlNet. For synthetic data generation, the prompts provided to ControlNet now include these captions, with under-represented data subgroups acting as a stylistic influence to generate synthetic images tailored to these specific subgroups.

% \item We demonstrate that fine-tuning existing semantic segmentation models by augmenting the original dataset not only improves the average performance of semantic segmentation models but also enhances the performance of these models on under-represented subgroups.

% \item Finally, we are the first to show that we can augment autonomous driving datasets with a blend of real and synthetic images without the need for additional expert data. Autonomous driving models fine-tuned on augmented datasets showed improved driving performance across various test subgroups.


% Our key contributions are summarised as follows:
% \begin{enumerate}
% \item We focus on generating synthetic scenarios conditioned on ground truth labels for under-represented subgroups by leveraging a state-of-the-art text-conditioned image generative model—ControlNet. Here, we ensure that the synthetic images retain essential semantics for subsequent fine-tuning of segmentation and autonomous planning models without requiring additional labels.

% \item We propose fine-tuning ControlNet with a text description of an image generated by a vision-language captioning model, LLaVA. Our experiments reveal that this approach improves the quality of images generated for downstream synthesis.

% \item Inspired by textual inversion, we propose fine-tuning ControlNet to generate synthetic data for different data subgroups through style prompting. To achieve this, we integrate captions generated by the vision captioning model LLaVA and identify data subgroups as a stylistic guide for fine-tuning ControlNet. For synthetic data generation, the prompts provided to ControlNet now include these captions, with under-represented data subgroups acting as a stylistic influence to generate synthetic images tailored to these specific subgroups.

% \item We demonstrate that fine-tuning existing semantic segmentation models by augmenting the original dataset not only improves the average performance of semantic segmentation models but also enhances the performance of these models on under-represented subgroups.

% \item Finally, we are the first to show that we can augment autonomous driving datasets with a blend of real and synthetic images without the need for additional expert data. Autonomous driving models fine-tuned on augmented datasets showed improved driving performance across various test subgroups.
% \end{enumerate}



% the compiled datasets such as the Waymo Open Dataset \cite{sun2020scalability}, are predominantly biased with over-represented subgroups, for instance, weather conditions such as sunny and clear weather. This results in a dataset bias toward certain scenarios and neglects various conditions in which autonomous vehicles would operate. In prior work, this imbalance has been shown to affect the performance of segmentation models \cite{kerim2022semantic}, control \cite{pmlr-v205-agarwal23b} and autonomous driving \cite{agarwal2023robust}.  

% Over the last decade, the autonomous driving (AD) sector has experienced remarkable advancements, with vehicle fleets collecting extensive driving data. This process has expanded data availability at an unprecedented scale. Despite this progress, the compiled datasets such as the Waymo Open Dataset \cite{sun2020scalability}, are predominantly biased with over-represented subgroups, for instance, weather conditions such as sunny and clear weather. This results in a dataset bias toward certain scenarios and neglects various conditions in which autonomous vehicles would operate. In prior work, this imbalance has been shown to affect the performance of segmentation models \cite{kerim2022semantic}, control \cite{pmlr-v205-agarwal23b} and autonomous driving \cite{agarwal2023robust}.  

% Assuming that these conditions or subgroups are defined by a human or obtained through an LLM, a key requirement for improving the generalization capabilities for semantic segmentation or AD over under-represented subgroups is to generate data for infrequently encountered data subgroups. While this is feasible given the expensive AV infrastructure for additional data collection \cite{akcin2023data}, the subsequent manual labeling process is expensive and time-consuming. This is especially true for tasks like semantic segmentation and end-to-end autonomous driving. To mitigate this imbalance for some data subgroups such as weather, synthetic datasets \cite{marathe2023t,marathe2023wedge} have been generated using Dalle-2 \cite{ramesh2022hierarchical}. However, these datasets still necessitate human-in-the-loop evaluation to verify the quality of annotations. Moreover, they fail to cover the wide range of conditions that vehicles may encounter, such as variations in lighting or time of day. Therefore, another key requirement for generating synthetic data is to prevent the need for subsequent human annotations for further training.  

% To address these challenges, we present \textcolor{red}{NAME OF METHOD} that presents a complete solution to improving the generalization capabilities of a model over under-represented subgroups of data. Our key contributions are summarised as follows:
% \begin{enumerate}
%     % \item We introduce a toolkit that facilitates the evaluation of semantic segmentation and autonomous driving models across various data subgroups, more specifically characterized by weather and day-light conditions. We assume that the set of test subgroups can be defined either manually or through a Large Language Model. We leverage CLIP to classify images within the test dataset according to these specified subgroups and evaluate the subgroup-specific performance of SOTA segmentation and autonomous driving models.
% \item We focus on generating synthetic scenarios conditioned on ground truth labels for under-represented subgroups by leveraging a state-of-the-art text-conditioned image generative model—ControlNet. Here, we ensure that the synthetic images retain essential semantics for subsequent fine-tuning of segmentation and autonomous planning models without requiring additional labels.

% \item We propose fine-tuning ControlNet with a text description of an image generated by a vision-language captioning model, LLaVA. Our experiments reveal that this approach improves the quality of images generated for downstream synthesis.

% \item Inspired by textual inversion, we propose fine-tuning ControlNet to generate synthetic data for different data subgroups through style prompting. To achieve this, we integrate captions generated by the vision captioning model LLaVA and identify data subgroups as a stylistic guide for fine-tuning ControlNet. For synthetic data generation, the prompts provided to ControlNet now include these captions, with under-represented data subgroups acting as a stylistic influence to generate synthetic images tailored to these specific subgroups.

% \item We demonstrate that fine-tuning existing semantic segmentation models by augmenting the original dataset not only improves the average performance of semantic segmentation models but also enhances the performance of these models on under-represented subgroups.

% \item Finally, we are the first to show that we can augment autonomous driving datasets with a blend of real and synthetic images without the need for additional expert data. Autonomous driving models fine-tuned on augmented datasets showed improved planning performance across various test conditions or subgroups.
% \end{enumerate}


%Our key control 

% Here we assume that these scenarios or test conditions can be described using natural language or text, or generated by a Large Language Model (LLM). First, we propose a simple algorithm to characterize the performance of a model over under-represented data subgroups. Second, we leverage
% ControlNet which utilizes semantic segmentation masks and natural language prompts  \cite{zhang2023adding} to generate synthetic images. We introduce modifications to With text conditioning, we can target synthesis specifically toward under-represented downstream test data subgroups - eg. weather or lighting - that we want to further test and improve semantic segmentation and autonomous driving models over. Beyond leveraging the versatility of stable diffusion models to improve the diversity of image content, our method also uses semantically rich and informative prompts to ensure the production of high-quality synthetic training samples.  Specifically, we generate high-quality textual prompts by leveraging the off-the-shelf image captioning models such as LLaVA \cite{liu2023visual} to caption real images based on the identified semantics in the image. The underrepresented data subgroups are added to the original caption as styles to constitute the prompts for downstream synthesis.



% In summary, our contributions can be summarised as follows:
% \begin{enumerate}
%     \item We introduce a toolkit that facilitates the evaluation of semantic segmentation and autonomous driving models across various data subgroups, more specifically characterized by weather and lighting conditions. These conditions can be defined either manually or through a Large Language Model, with CLIP used to classify images within the dataset according to these specified conditions.
%     \item The toolbox aids in pinpointing the specific data subgroups where the model’s performance is sub-optimal and focuses on generating synthetic scenarios tailored to those conditions by leveraging a state-of-the-art text-conditioned image generative model- ControlNet. Here we ensure that the synthetic images retain essential semantics for the subsequent fine-tuning of segmentation and autonomous planning models without the need for additional labeled data.
%     \item Additionally, we propose a fine-tuning mechanism, inspired by textual inversion, for ControlNet that is tailored towards synthetic data generation over the identified data subgroups. This fine-tuning process supervises ControlNet by enhancing the text descriptions used for the conditional synthesis. To achieve this, we integrate captions generated by the vision captioning model LLaVA, and the identified data subgroup as a stylistic guide, for generating the supervisory image. Consequently, the prompts provided to ControlNet for data generation now include these captions, with the targeted data subgroup acting as a stylistic influence, thereby enabling the creation of synthetic images tailored to these specific conditions
%     \item Finally, we show that fine-tuning existing segmentation and autonomous driving models with a blend of real and synthetic images, conditioned on ground truth semantic masks and text prompts, significantly surpasses the performance of models trained exclusively on original dataset images across all test subgroups.
    
% \end{enumerate}
% proposed toolbox enables testing semantic segmentation to different test conditions in natural language when training models for vision or control tasks in autonomous driving for instance weather. These tools will identify and highlight the specific conditions where the model’s performance is sub-optimal and focus on generating scenarios tailored to those conditions.
% Finally, we finetune existing segmentation models using the synthetic data. Ablations reveal that fine-tuning segmentation models such as Mask2Former with a mixture of real and synthetic images marginally outperform those that are fine-tuned purely on synthetic or original images. Finally, we show that the generated synthetic images improve performance of the models over the downstream test conditions for instance weather and daylight conditions.
% \begin{table*}[t]
%   \centering
% \begin{minipage}[b]{0.45\linewidth}
%     \centering
%   \caption{Training Dataset Distribution
%   over Environmental Conditions consisting 39618 images }
%   \label{tab:conditions}
%   \begin{tabular}{ccc}
%     \toprule
%     Day Conditions & Environmental Conditions & Percentage \\
%     \midrule
%     Day & Clear & 62.64 \\
%     Day & Rainy &  17.26 \\
%     Day & Cloudy& 5.66  \\
%      \midrule
%     Dawn/Dusk & Clear & 6.04\\
%     Dawn/Dusk & Rainy & 1.81\\
%     Dawn/Dusk & Cloudy & 0.72\\
%      \midrule
%     Night & Clear & 1.85\\
%     Night & Rainy & 3.34 \\
%     Night & Cloudy& 0.64 \\
%     \bottomrule
%   \end{tabular}
% \end{minipage}     
% \hfill
% \begin{minipage}[b]{0.45\linewidth}
%   \centering
%   \caption{Testing Dataset Distribution
%   over Environmental Conditions consisting 5970 images}
%   \label{tab:conditions}
%   \begin{tabular}{ccc}
%     \toprule
%     Day Conditions & Environmental Conditions & Percentage \\
%     Day & Clear & 72.55 \\
%     Day & Rainy &  7.18 \\
%     Day & Cloudy& 2.22  \\
%      \midrule
%     Dawn/Dusk & Clear & 3.67\\
%     Dawn/Dusk & Rainy & 5.56\\
%     Dawn/Dusk & Cloudy & 0.81\\
%      \midrule
%     Night & Clear & 1.98\\
%     Night & Rainy & 5.1 \\
%     Night & Cloudy& 0.82 \\
%     \bottomrule
%   \end{tabular}
%   \end{minipage}
% \end{table*}


==> sections/new_intro_oguzhan.tex <==
\section{Introduction}

Autonomous driving (AD) has the potential to transform transportation, making it safer and more efficient by reducing human error and optimizing traffic flow. Over the last decade, advancements in AD have been fueled by the availability of massive amounts of driving data collected daily from vehicle fleets~\cite{liu2024surveyautonomousdrivingdatasets}. Companies such as Waymo and Tesla generate and process \textbf{millions of miles} of driving data each year, producing \textbf{terabytes of visual data} to power deep neural networks (DNNs) for critical tasks like object detection, semantic segmentation, and end-to-end (E2E) driving control. These advances have been crucial in pushing AD systems closer to real-world deployment. 

One of the primary challenges in AD lies in the \textit{imbalance of environmental conditions} in these datasets. Large-scale datasets, such as Waymo Open~\cite{sun2020scalability} and DeepDrive~\cite{yu2020bdd100k}, primarily capture common scenarios, such as sunny or clear weather, while under-representing critical but rarer conditions like nighttime or rainy weather. For example, only \textbf{0.1\% of Waymo’s data} includes nighttime scenes, leading to a significant bias that can impair AD models’ performance in such conditions. This imbalance has measurable impacts: in semantic segmentation tasks, models like Mask2Former~\cite{cheng2022masked} experience a \textbf{40\% performance drop} on samples taken in rainy or nighttime settings compared to daytime, clear-weather data. Similarly, E2E driving models struggle with rare conditions, potentially jeopardizing reliability in real-world deployment.

A common approach in the industry is to collect additional data targeting these under-represented scenarios. However, acquiring diverse, high-quality data is resource-intensive, requiring complex sensor setups, expansive fleet deployment, and extensive manual annotation. While recent simulation environments like CARLA~\cite{Dosovitskiy17} aim to alleviate some of this burden by generating synthetic data under controlled conditions, such tools still demand significant computational resources and may lack the environmental diversity and fidelity needed to train robust models. This creates a pressing need for scalable, intelligent data augmentation methods that can efficiently generate realistic data for AD applications.

Many research efforts focus on developing new model architectures to improve AD performance, especially in challenging conditions. However, high-quality \textit{data augmentation} is equally essential and complementary to new architectural developments, as it enables models to generalize across diverse conditions, making them more robust in practical applications~\cite{li2024datacentric}. This motivates the need for advanced data augmentation techniques, which are essential for achieving better performance across AD tasks such as semantic segmentation and E2E driving.

To address these challenges, we propose \textbf{SynDiff-AD}, a novel data augmentation pipeline that leverages generative models, specifically latent diffusion models (LDMs), to create realistic synthetic data for under-represented conditions. Our approach (Fig.~\ref{fig:intro_fig}) takes existing data samples and \textit{transforms their environmental conditions}—for instance, converting sunny scenes into rainy or nighttime scenes—to expand the diversity of rare scenarios in the dataset. By preserving key semantic annotations, such as object bounding boxes and segmentation masks, SynDiff-AD enables the creation of balanced datasets without incurring the costs of additional manual labeling or high-fidelity simulation setups.

Furthermore, SynDiff-AD introduces an innovative prompting scheme inspired by \textit{textual inversion}, leveraging LLaVA~\cite{zhang2023adding}, a vision-language captioning model. By generating detailed descriptions of over-represented samples and strategically modifying them to represent under-represented conditions, we guide our model to synthesize data that is both semantically rich and tailored to AD training needs. This approach ensures that the generated data aligns closely with real-world distributions, improving AD models' robustness in diverse conditions.

Our key contributions are as follows:
\begin{enumerate}
    \item \textbf{Conditional LDM-based Augmentation}: We introduce SynDiff-AD, a pipeline that generates samples for under-represented conditions while preserving the semantic structure of the original data.
    \item \textbf{Novel Prompting Scheme for Synthetic Data}: Inspired by textual inversion, our prompting approach leverages vision-language captions to guide synthetic data generation towards rare conditions, effectively balancing datasets across diverse environmental scenarios.
    \item \textbf{Empirical Performance Improvements}: Fine-tuning models on SynDiff-AD-augmented datasets results in performance gains of up to 3.6\% for semantic segmentation and 20\% for AD models in rare scenarios, demonstrating the pipeline’s effectiveness in enhancing model robustness and generalizability.
\end{enumerate}
